Self-supervised Knowledge Triplet Learning for Zero-shot Question Answering

The aim of all Question Answering (QA) systems is to be able to generalize to unseen questions. Current supervised methods are reliant on expensive data annotation. Moreover, such annotations can introduce unintended annotator bias which makes systems focus more on the bias than the actual task. In this work, we propose Knowledge Triplet Learning (KTL), a self-supervised task over knowledge graphs. We propose heuristics to create synthetic graphs for commonsense and scientific knowledge. We propose methods of how to use KTL to perform zero-shot QA and our experiments show considerable improvements over large pre-trained transformer models.

==> name.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% \begin{table}[t]
% \small
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}ccccc@{}}
% \toprule
% \textbf{Type}                       & \textbf{Model}       & \textbf{Train-Val} & \textbf{Val}  & \textbf{Deviation} \\ \midrule
% \multirow{4}{*}{Baselines} & Majority    & 33.5      & 33.6 &       \\ %\cmidrule(l){2-5} 
%                           & GPT2-L      & 41.3      & 41.1 &       \\ %\cmidrule(l){2-5} 
%                           & RoBERTa     & 33.6      & 33.4 &       \\ %\cmidrule(l){2-5} 
%                           & RoBERTa-MLM & 36.4      & 34.3 & +/-0.8 \\ %\midrule
% \citeauthor{shwartz2020unsupervised}             & Self-Talk   & 46.5      & 46.2 &       \\ %\midrule
% \multirow{4}{*}{Ours}      & KRL-L2      & 43.2      & 43.8 & +/-0.3 \\ %\cmidrule(l){2-5} 
%                           & KRL-NCE-L2  & 46.4      & 46.2 & +/-0.2 \\ %\cmidrule(l){2-5} 
%                           & KRL-NCE-Cos & 46.6      & 46.4 & +/-0.2 \\ %\cmidrule(l){2-5} 
%                           & SMLM        & \textbf{48.7}      & \textbf{48.5} & +/-0.4 \\ %\midrule
% Supervised                 & Sup RoBERTa &           & 76.6 &    +/-0.6   \\ %\midrule
%                           & Human       &           & 86.9 &       \\ \bottomrule
% \end{tabular}
% }
% \caption{Accuracy comparison with our baseline models on the SocialIQA dataset. We compare the models on the  Zero-shot task. We compare them on both Train-Val split (35k) and the Validation split (2k), to enable measuring better statistical significance. }
% \label{tab:my-table}
% \end{table}


% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[h]
% \centering
% \small
% \begin{tabular}{@{}lll@{}}
% \toprule
% \textbf{Model}       & \textbf{Val}   & \textbf{Deviation}   \\ \midrule
% RoBERTa     & 44.4  & +/-1.2 \\ \midrule
% RoBERTa+MLM & 46.8  & +/-0.6  \\ \midrule
% KRL-NCE-Cos & 58.6  & +/-0.8 \\ \midrule
% SMLM        & \textbf{69.1} & +/-0.4  \\ \bottomrule
% \end{tabular}
% \caption{Accuracy comparison on Few-shot Question Answering. We re-use our Transformer encoder for the few-shot task with only 8 \% train samples. }
% \label{tab:fewshot}
% \end{table}


% % \subsection{SocialIQA}
% % This dataset is about reasoning over social interactions and the implications of social events. Each instance in this dataset contains a context $C$ which is a social situation, a question $Q$ about this situation, and three answer options. There are several question types that are derived from the different ATOMIC inference dimensions, such as Intent, Effect, Attributes, etc. There are 33,410 training samples and 1954 validation samples, with a withheld test set.

% % Though this dataset is derived from the ATOMIC knowledge graph, the fact triples present in the graph are considerably different than the context, question and answers present in the dataset as they are crowdsourced. The average length of the event description in ATOMIC is 10, max length is 18. Whereas in SocialIQA the average length is 36 and max is 124. This shows the varied type of questions present in SocialIQA, and possess a much more challenge in unsupervised learning.

% % \subsection{aNLI}
% % \subsection{CommonsenseQA}
% % \subsection{ARC, OpenBookQA and QASC}

% % \section{Knowledge Graph Generation}


% Table \ref{tab:my-table} shows our evaluation and baseline comparisons for the zero-shot task. We can observe our KTL trained models perform significantly well compared to the baselines. When comparing the different KRL models, the NCELoss with Cosine similarity performs the best. This might be due to the additional supervision provided by the negative samples as the L2Loss model only tries to minimize the two projections. When comparing different KTL instantiations we can see the SMLM model performs the best overall but has a slightly higher deviation. We are analyzing our model to understand this phenomenon better. Our KRL model does perform equal to the current state-of-the-art model, Self-Talk \cite{shwartz2020unsupervised} which uses two GPT type models. Our models have half the parameters compared to Self-Talk. We also compare our model on the entire Train-Val set of 35,364 questions in the zero-shot setting to better gauge the statistical significance of the different model accuracies. 



% Table \ref{tab:fewshot} compares the different pre-trained Transformer encoders in the few-shot question answering task. We randomly sample three sets of 2,400 samples as training data from the training set. We train our models on these three sets and measure the validation set accuracy. We can see the Transformer encoder trained on KTL perform significantly better than the baseline models in this setting. This shows that encoders trained on KTL are able to learn with a few samples. We plan to continue analyzing our models and evaluate the KTL framework on different datasets. 
